Detecting and Correcting for Label Shift with Black Box Predictors

Faced with distribution shift between training and test set, we wish to detect and quantify the shift, and to correct our classifiers without test set labels. Motivated by medical diagnosis, where diseases (targets) cause symptoms (observations), we focus on label shift, where the label marginal $p(y)$ changes but the conditional $p(x| y)$ does not. We propose Black Box Shift Estimation (BBSE) to estimate the test distribution $p(y)$. BBSE exploits arbitrary black box predictors to reduce dimensionality prior to shift correction. While better predictors give tighter estimates, BBSE works even when predictors are biased, inaccurate, or uncalibrated, so long as their confusion matrices are invertible. We prove BBSE's consistency, bound its error, and introduce a statistical test that uses BBSE to detect shift. We also leverage BBSE to correct classifiers. Experiments demonstrate accurate estimates and improved prediction, even on high-dimensional datasets of natural images.

==> sections/generalizations.tex <==
%!TEX root = ../labelshift.tex

\subsection{Handling continuous labels with kernel density estimation}
Equation \eqref{eq:main_idea}  and Lemma~\ref{lem:matching_confusion}  also apply to the case when the label is continuous. For example, in the regression problems $\cY$ is typically a compact subset of $\R$.  In this section, we consider $\cY = [0,1]$ and work out an algorithm to estimate the importance weight 
$$\vct w := \left[\frac{q(y_1)}{p(y_1)}, ..., \frac{q(y_n)}{p(y_n)}\right],$$
 and more generally, estimating the function $w(y) = \frac{q(y)}{p(y)}$ for each $y\in \cY$.
 
\paragraph{From function to sequence.} Let $\Phi = \{\phi_i\}_{i\in \mathbb{Z}_+}$ and  $\varPhi = \{\varphi_i\}_{i\in \mathbb{Z}_+}$ be collections of basis of functions $\cY\rightarrow \R$ supported on $\cY$, assume $\vct v$ and $\vct u$ are the vector of coefficients such that
$$
q(\hat{y}) = \sum_i \phi_i(\hat{y}) v_i  =    \Phi \vct v
$$
$$
w(y) = \frac{q(y)}{p(y)}  = \sum_{j} \varphi_j(y) u_j =\varPhi \vct u
$$
Similarly, let $\Psi = \{\psi_i\}_{i\in\mathbb{Z}_+}$ be a collection basis functions $\cY^2 \rightarrow \R$ and coefficient vector $\vct c$ obeys that 
$$
p(\hat{y},y)  = \sum_{l}\psi_lc_l =   \Psi \vct c.
$$
Then for every $\hat{y}$, we can rewrite equation \eqref{eq:main_idea}  as
$$
\Phi(\hat{y}) \vct v  = \int_{y\in\cY}  [\Psi(\hat{y},y) \vct c ]  [\varPhi(y) \vct u]  dy  
$$
which holds for every $\hat{y}$ and the task of estimating function $w(y)$ reduces to estimate the coefficient vector $\vct u$. 
We can further replace the above expression in a more linear algebraic form as follows
\begin{equation}\label{eq:moment_eq}
\Phi(\hat{y}) \vct v  = \text{Vol}(\cY) \left\langle \Phi(\hat{y},\cdot) \vct c,   \varPhi(\cdot) \vct u  \right\rangle   =    \vct c^T[\Psi(\hat{y},\cdot)^T\varPhi(\cdot)] \vct u.
\end{equation}
Note that the left hand side is a number in $\R$, $[\Psi(\hat{y},\cdot)^T\varPhi(\cdot)] $ is a matrix in $\R^{|\Psi|\times |\varPhi|}$. Combining these equations for a sequence of $\hat{y}$,  this becomes a system of linear equations. 

\paragraph{Regularized moment-matching estimator.}
In practice, we can estimate $q(\hat{y})$ and $p(\hat{y},y)$ using kernel density estimator in $L_2$ with rate $O(m^{-\frac{2v}{2v+1}})$ and  $O(n^{-\frac{2v}{2v+2}})$ respectively when we assume the density $q(\hat{y})$ and $p(\hat{y},y)$ are $v$th order continuously differentiable (Cite standard nonparametric statistics textbook).

In particular, these kernel density estimators can be written as linear combination of a \emph{finite} basis functions --- often``bump''-like highly kernel functions centered at the observed locations. In other word, $\Phi$ contains $m$ such  functions centered at $f(\vct x'_1),...,f(\vct x'_m)$, and $\Psi$ contains $n$ such functions centered at $(f(x_1), y_1),...,(f(x_n),y_n)$. Now we need to choose an appropriate basis function $\varPhi$ for $q(y)$ on the right hand side. One natural choice is to simply take $\varPhi = \Phi$ so $\hat{\vct u}\in \R^m$. 

By evaluating these functions at a sequence of locations, e.g., 
$$\cT = \{f(\vct x_1),...,f(\vct x_n), f(\vct x'_1),...,f(\vct x'_m)\} \subset \cY,$$
 we are able to construct an estimator of $\vct u$ analogous to what we have in the discrete case:
\begin{equation}\label{eq:continuous_estimator}
\hat{\vct u}   =    (\widehat{A}^T\widehat{A} + \lambda I)^{-1} \widehat{A} \Phi \hat{\vct v} 
\end{equation}
where $\lambda>0$ is an appropriately chosen  tuning parameter. We overload the notation and use $\Phi$ to denote the matrix where its $i$th column is in $\R^{m+n}$ and it contains the evaluation of $\phi_i$ at all points in $\cT$. Moreover, 
$\widehat{A}\in\R^{(m+n)\times k}$ is the matrix where 
$$
\widehat{A}_{i,j}  = \sum_{l=1}^n \hat{c}_l \psi_l(t_i,\cdot)^T\phi_j(\cdot)  \text{Vol}(\cY)  = \sum_{l=1}^{n} \hat{c}_l  \int_{y\in \cY} \psi_l(t_i,y)\phi_j(y)   dy.
$$
The integrals above can then be evaluated either analytically or through numerical methods and the solution to \eqref{eq:continuous_estimator} gives us
$$\hat{w}(\cdot)  =   \sum_{i=1}^k  \varphi_i (\cdot) \hat{u}_i,$$
which can then be used as a good approximation of the importance weights.  Detailed  analysis of consistency and finite sample error bound are omitted for the interest of space. 

Lastly, we note that this strictly generalizes the discrete case we presented in Section~\ref{sec:theory}, which corresponds to taking the basis functions to be indicators supported on the discrete set. 


\subsection{Estimating the RKHS embedding of $q(y)$ directly.}
Sometimes we are interested in finding the RKHS embedding of the distribution $q(y)$, which is defined as
$$
\vct \mu_Q(y) = \E_Q k(y,\cdot)
$$
for a kernel function $k$ satisfying the Mercer's condition. Such embedding are used conducting statistical tests, graphical model inferences, learning with label proportions, ecological inference and so on. The techniques in paper provides one way to construct an estimator of $\vct \mu_Q(y)$ without observing samples from $q(y)$.

%Equation \eqref{eq:main_idea} 
The idea is to use the kernel embedding of condition distributions as was developed in \citet{song2013kernel}, where the cross-covariance operators are defined as ${\mat C}_Q(\hat{y} | y)  :=  \E_Q[ k(\hat{y},\cdot) |  y]$. The (kernel) Bayes rule suggests that
$$
\vct \mu_Q(\hat{y})   =  {\mat C}_Q(\hat{y} | y)  \vct \mu_Q(y).
$$
Note that under the label-shift assumption, ${\mat C}_Q(\hat{y} | y)  = {\mat C}_P(\hat{y} | y)$ therefore can be estimated. This allows us to directly estimate $ \vct \mu_Q(y)$ by matching moments and solving a kernel ridge regression the plug-in estimates of $\vct \mu_Q(\hat{y})$ and ${\mat C}_P(\hat{y} | y)$. It can be worked out that thanks to the ``kernel-trick'' we do not need to explicitly deal with infinite dimensional objects.  
Details are omitted. 


\begin{comment}
can also be interpreted more generally as the functions and conditional expectation operators in a reproducing kernel Hilbert space (RKHS). Let the associated feature maps be $\phi: \cY \rightarrow \cH$.  
In particular, $\vct \mu_Q(y) := \E_Q \phi(y),  \vct \mu_Q(\hat{y}) := \E_Q\phi(f(\vct x))$ are the kernel mean embedding of the distribution defined on $\cY$, and linear operator ${\mat C}_{\hat{y} |y} =  \vct \E_Q[ \phi(y)| \phi(f(\vct x)) ] $ is the kernel embedding of the conditional distributions. 

Using kernel ridge regression, we can estimate $ \mu_Q(y)$ by solving a linear system of equations with the plug-in estimate of ${\mat C}(\hat{y} | y)  $ and $\vct \mu_Q(\hat{y}) $. As we will see, this leads to a natural hypothesis test on whether there is a label shift for continuous $\cY$.

This however, does not provide us a way to correct label shift. We can do it using any nonparametric regression estimator, e.g., smoothing kernels. In particular, this will be very helpful if $\cY = [0,1]$. What we do is basically estimating the bivariate density $p(\hat{y},y)$ and $q(\hat{y})$ separately. 

It can be written that $\hat{p}_P(\hat{y},y) =  \sum_i k_{2d}[i](\hat{y},y) \gamma_i $  and $\hat{p}_Q(\hat{y})  =  \sum_i  k_{1d}[i](\hat{y}) \alpha_i $. Basically we can rewrite \eqref{eq:main_idea2} by
$$
\sum_i  k_{1d}[i](\hat{y}) \alpha_i   =  \int_{y}\sum_i k_{2d}[i](\hat{y},y) \gamma_i  \beta(y) dy.
$$
If we linearly represent $\beta(y)  =  \sum_i  k_{1d}[i](y) \beta_i $, the above equation becomes effectively
$$
\sum_i  k_{1d}[i](\hat{y}) \alpha_i   =  \int_{y}\sum_i k_{2d}[i](\hat{y},y) \gamma_i  \sum_j  k_{1d}[i](y) \beta_j dy  =    \sum_j  \sum_i \gamma_i   \beta_j  \int_y k_{2d}[i](\hat{y},y) k_{1d}[i](y) dy .
$$

This is a linear system of equation for coefficient vector $\vct \beta \in \R^n$.
$$
K\vct \alpha  =   \tilde{K}  \diag(\vct \gamma) \vct \beta 
$$
where $K\in \R^{m\times m}$ is the evaluation of the basis functions at the observed sequence of $m$ points. $\tilde{K}\in \R^{m\times n}$ is the evaluation of the  basis function $ \int_y k_{2d}[i](\hat{y},y) k_{1d}[i](y) dy $ for $i=1,...,n$ evaluated at the same $m$ locations.

The difference from the RKHS approach is that now we have an explicit basis representation that we can use to evaluate the propensity scores. 
\end{comment}


\subsection{Weakening Label-Shift with latent representations and GAN}
\red{We should perhaps reserve this part for NIPS, if some intern is able to do the experiments. But it's a good idea at least.}

Consider the case when $x|y$ also changes but there are some hidden states $z|y$ that remains unchanged and $x|z$ got rendered differently.

An example is the following: $y => \text{Graphics Engine generated } x$ in the training data.

In test time:
$y => \text{Real-life images} x$.

Feature extractors that learn $x => z$ for both synthetically generated $x$ and real-life $x$ and somehow match their internal representation. 


